Catalytic Role Of Noise And Necessity Of Inductive Biases In The Emergence Of Compositional Communication

Communication is compositional if complex signals can be represented as a combination of simpler subparts. In this paper, we theoretically show that inductive biases on both the training framework and the data are needed to develop a compositional communication. Moreover, we prove that compositionality spontaneously arises in the signaling games, where agents communicate over a noisy channel. We experimentally confirm that a range of noise levels, which depends on the model and the data, indeed promotes compositionality. Finally, we provide a comprehensive study of this dependence and report results in terms of recently studied compositionality metrics: topographical similarity, conflict count, and context independence.

==> images/baseline_obverter.tex <==
\begin{tabular}{l|ccccc}
\toprule
noise &                                               topo &                                               conf &                                               cont &                                                pos &                                                acc \\ \midrule
\midrule
0.00 &   \makecell{$0.71$ \\ \scriptsize{$[0.67, 0.74]$}} &   \makecell{$5.54$ \\ \scriptsize{$[4.78, 6.32]$}} &   \makecell{$0.15$ \\ \scriptsize{$[0.15, 0.16]$}} &   \makecell{$0.45$ \\ \scriptsize{$[0.40, 0.50]$}} &   \makecell{$0.95$ \\ \scriptsize{$[0.94, 0.97]$}} \\ \midrule
0.02 &   \makecell{$0.74$ \\ \scriptsize{$[0.72, 0.76]$}} &   \makecell{$6.15$ \\ \scriptsize{$[5.39, 6.93]$}} &   \makecell{$0.15$ \\ \scriptsize{$[0.15, 0.16]$}} &   \makecell{$0.38$ \\ \scriptsize{$[0.33, 0.43]$}} &   \makecell{$0.98$ \\ \scriptsize{$[0.98, 0.98]$}} \\ \midrule
0.04 &   \makecell{$0.78$ \\ \scriptsize{$[0.76, 0.80]$}} &   \makecell{$5.19$ \\ \scriptsize{$[4.43, 5.99]$}} &   \makecell{$0.16$ \\ \scriptsize{$[0.15, 0.16]$}} &   \makecell{$0.45$ \\ \scriptsize{$[0.39, 0.50]$}} &   \makecell{$0.97$ \\ \scriptsize{$[0.97, 0.98]$}} \\ \midrule
0.06 &   \makecell{$0.79$ \\ \scriptsize{$[0.77, 0.82]$}} &   \makecell{$4.36$ \\ \scriptsize{$[3.63, 5.11]$}} &   \makecell{$0.16$ \\ \scriptsize{$[0.16, 0.17]$}} &   \makecell{$0.52$ \\ \scriptsize{$[0.46, 0.57]$}} &   \makecell{$0.92$ \\ \scriptsize{$[0.90, 0.94]$}} \\ \midrule
0.08 &   \makecell{$0.83$ \\ \scriptsize{$[0.80, 0.85]$}} &   \makecell{$3.58$ \\ \scriptsize{$[2.87, 4.34]$}} &   \makecell{$0.17$ \\ \scriptsize{$[0.17, 0.18]$}} &   \makecell{$0.59$ \\ \scriptsize{$[0.53, 0.65]$}} &   \makecell{$0.91$ \\ \scriptsize{$[0.89, 0.94]$}} \\ \midrule
0.10 &   \makecell{$0.85$ \\ \scriptsize{$[0.83, 0.88]$}} &   \makecell{$3.30$ \\ \scriptsize{$[2.54, 4.07]$}} &   \makecell{$0.18$ \\ \scriptsize{$[0.17, 0.18]$}} &   \makecell{$0.64$ \\ \scriptsize{$[0.58, 0.70]$}} &   \makecell{$0.91$ \\ \scriptsize{$[0.89, 0.93]$}} \\ \midrule
0.12 &   \makecell{$0.86$ \\ \scriptsize{$[0.84, 0.89]$}} &   \makecell{$3.14$ \\ \scriptsize{$[2.37, 3.96]$}} &   \makecell{$0.18$ \\ \scriptsize{$[0.18, 0.19]$}} &   \makecell{$0.70$ \\ \scriptsize{$[0.64, 0.76]$}} &   \makecell{$0.90$ \\ \scriptsize{$[0.87, 0.92]$}} \\ \midrule
0.14 &   \makecell{$0.86$ \\ \scriptsize{$[0.83, 0.88]$}} &   \makecell{$3.50$ \\ \scriptsize{$[2.70, 4.34]$}} &   \makecell{$0.18$ \\ \scriptsize{$[0.18, 0.19]$}} &   \makecell{$0.69$ \\ \scriptsize{$[0.62, 0.75]$}} &   \makecell{$0.88$ \\ \scriptsize{$[0.86, 0.90]$}} \\ \midrule
0.16 &   \makecell{$0.86$ \\ \scriptsize{$[0.83, 0.88]$}} &   \makecell{$3.87$ \\ \scriptsize{$[3.02, 4.72]$}} &   \makecell{$0.18$ \\ \scriptsize{$[0.17, 0.19]$}} &   \makecell{$0.67$ \\ \scriptsize{$[0.60, 0.73]$}} &   \makecell{$0.87$ \\ \scriptsize{$[0.85, 0.89]$}} \\ \midrule
0.18 &   \makecell{$0.82$ \\ \scriptsize{$[0.80, 0.85]$}} &   \makecell{$4.73$ \\ \scriptsize{$[3.91, 5.57]$}} &   \makecell{$0.17$ \\ \scriptsize{$[0.16, 0.18]$}} &   \makecell{$0.63$ \\ \scriptsize{$[0.58, 0.69]$}} &   \makecell{$0.82$ \\ \scriptsize{$[0.79, 0.85]$}} \\ \midrule
0.20 &   \makecell{$0.80$ \\ \scriptsize{$[0.78, 0.82]$}} &   \makecell{$6.34$ \\ \scriptsize{$[5.44, 7.23]$}} &   \makecell{$0.16$ \\ \scriptsize{$[0.16, 0.17]$}} &   \makecell{$0.60$ \\ \scriptsize{$[0.54, 0.65]$}} &   \makecell{$0.75$ \\ \scriptsize{$[0.72, 0.78]$}} \\ \midrule
0.22 &   \makecell{$0.78$ \\ \scriptsize{$[0.77, 0.80]$}} &   \makecell{$7.22$ \\ \scriptsize{$[6.41, 8.03]$}} &   \makecell{$0.16$ \\ \scriptsize{$[0.15, 0.17]$}} &   \makecell{$0.60$ \\ \scriptsize{$[0.55, 0.65]$}} &   \makecell{$0.69$ \\ \scriptsize{$[0.65, 0.72]$}} \\ \midrule
0.24 &   \makecell{$0.76$ \\ \scriptsize{$[0.75, 0.78]$}} &   \makecell{$7.66$ \\ \scriptsize{$[6.98, 8.31]$}} &   \makecell{$0.16$ \\ \scriptsize{$[0.15, 0.16]$}} &   \makecell{$0.62$ \\ \scriptsize{$[0.57, 0.66]$}} &   \makecell{$0.62$ \\ \scriptsize{$[0.59, 0.65]$}} \\ \midrule
0.26 &   \makecell{$0.74$ \\ \scriptsize{$[0.73, 0.76]$}} &   \makecell{$8.42$ \\ \scriptsize{$[7.91, 8.92]$}} &   \makecell{$0.15$ \\ \scriptsize{$[0.14, 0.16]$}} &   \makecell{$0.59$ \\ \scriptsize{$[0.55, 0.63]$}} &   \makecell{$0.57$ \\ \scriptsize{$[0.55, 0.60]$}} \\ \midrule
0.28 &   \makecell{$0.74$ \\ \scriptsize{$[0.73, 0.75]$}} &   \makecell{$8.81$ \\ \scriptsize{$[8.32, 9.28]$}} &   \makecell{$0.15$ \\ \scriptsize{$[0.14, 0.16]$}} &   \makecell{$0.60$ \\ \scriptsize{$[0.57, 0.64]$}} &   \makecell{$0.54$ \\ \scriptsize{$[0.52, 0.57]$}} \\ \midrule
0.30 &   \makecell{$0.73$ \\ \scriptsize{$[0.72, 0.74]$}} &   \makecell{$8.94$ \\ \scriptsize{$[8.48, 9.40]$}} &   \makecell{$0.15$ \\ \scriptsize{$[0.14, 0.16]$}} &   \makecell{$0.64$ \\ \scriptsize{$[0.60, 0.67]$}} &   \makecell{$0.51$ \\ \scriptsize{$[0.49, 0.53]$}} \\ \midrule
\bottomrule
\end{tabular}

